Network-aware Recommendations in the Wild: Methodology, Realistic Evaluations, Experiments

Joint caching and recommendation has been recently proposed as a new paradigm for increasing the efficiency of mobile edge caching. Early findings demonstrate significant gains for the network performance. However, previous works evaluated the proposed schemes exclusively on simulation environments. Hence, it still remains uncertain whether the claimed benefits would change in real settings. In this paper, we propose a methodology that enables to evaluate joint network and recommendation schemes in real content services by only using publicly available information. We apply our methodology to the YouTube service, and conduct extensive measurements to investigate the potential performance gains. Our results show that significant gains can be achieved in practice; e.g., 8 to 10 times increase in the cache hit ratio from cache-aware recommendations. Finally, we build an experimental testbed and conduct experiments with real users; we make available our code and datasets to facilitate further research. To our best knowledge, this is the first realistic evaluation (over a real service, with real measurements and user experiments) of the joint caching and recommendations paradigm. Our findings provide experimental evidence for the feasibility and benefits of this paradigm, validate assumptions of previous works, and provide insights that can drive future research.

==> Introduction_BACKUP_07Apr2020.tex <==
Mobile Edge Caching (MEC) is one of the key technologies for 5G networks~\cite{MEC:white} that can reduce latency of service delivery and offload traffic from backhaul links. In MEC, caches are located at the edge of the mobile network (e.g., base stations), and thus have limited capacity and serve small --and frequently changing-- user populations~\cite{Paschos-infocom2016}. These factors, despite the advances in caching policies~\cite{Paschos-infocom2016} or delivery techniques~\cite{femto}, limit the possible gains from MEC: capacity is a tiny fraction of today's content catalogs, and traffic is highly variable; hence, a large number of user requests is for non-cached contents, i.e., not served in the edge.

A recently proposed solution for increasing the efficiency of MEC is jointly caching and recommending content~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching,giannakas-wowmom-2018}. Recommendation Systems (RS) are integrated in many popular services (e.g., YouTube, Netflix) and significantly affect the user demand~\cite{RecImpact-IMC10, gomez2016netflix}. Therefore, steering recommendations towards cached contents, can significantly increase the cache hit ratio, even with small caches or populations.%~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching,giannakas-wowmom-2018}.

However, joint caching and recommendation requires collaboration between network operators and Content Providers (CPs). This might be challenging, due to the different scope of these entities, and the constraints of current network protocols and architectures. For example, CPs encrypt traffic (e.g., https) and do not typically share user-related information~\cite{leguay2017cryptocache}. 

To bridge this gap, we propose an approach that is applicable in today's networks: the network operator leverages the information made available by the RS, and, based on this, provides \textit{independently of the CP} high-quality and cache-friendly recommendations that increase the efficiency of MEC. Specifically, we consider the YouTube service, and design a system/application that (i) obtains video relations from the YouTube API, based on which (ii) it builds extended lists of directly and indirectly related videos, and (iii) carefully steers initial recommendations --and thus user demand-- towards cached videos. These operations can take place without any tight collaboration with the CP, thus facilitating the application of joint caching and recommendation approaches by network operators (or other entities), without any need for modifications in architectures or protocols.


%\vassilis{We need to state here some of our quantitative results, in the form e.g., of CHR percentages. It will make the contribution stronger and will trigger the reader into proceeding.}
Our contributions are summarized as follows\footnote{\blue{A preliminary version of our work, appears in~\cite{kastanakis-cabaret-mecomm-2018}.}}:
%\vspace{-0.5\baselineskip}
\begin{itemize}[leftmargin=*]
\item We propose an approach that enables joint caching and recommendation, without requiring collaboration between network operators and CPs (\secref{sec:overview}). 
\item We design an algorithm (named \ourAlgo) that leverages available information provided by a RS, and returns cache-aware recommendations (\secref{sec:recommendation}).
\item We perform extensive measurements and evaluation over the YouTube service. Our results show that significant caching gains can be achieved in practice; even in conservative scenarios, our approach increases the cache hit ratio by a factor of 8 to 10 (\secref{sec:measurements}). \blue{To our best knowledge, this is the first evaluation of a joint caching and recommendation approach in a real service and with realistic traffic.}
\item We analytically study the problem of caching optimization under recommendations from \ourAlgo, and propose an approximation algorithm. We show that when caching is controlled by the network operator, an extra 2 times increase in the cache hit ratio can be achieved (\secref{sec:joint}). 
\item \blue{We build an experimental testbed and conduct experiments with \textit{real users} to (i) test the performance of \ourAlgo in practice, and (ii) verify to what extend the assumptions made hold in practice with real users (\secref{sec:experiments}). We are the first to test the concept of joint caching and recommendations with real user experiments. Moreover, we publish the collected dataset and open-source the code of the testbed (which is generic and enables researchers to design and conduct their own experiments either with \ourAlgo or with any other algorithm they implement.} 
\end{itemize}
\blue{Finally, we provide an overview of related work (\secref{sec:related}) and conclude our paper (\secref{sec:conclusions}).}


As a last remark, we would like to stress that while in this paper we focus on the YouTube service, which provides a public API, our approach can be extended to other video/radio services (e.g., Neflix, Vimeo, Spotify, Pandora) as well, e.g., using offline crawling processes (in case APIs are not available) for discovering content relations. 

%\blue{The paper is structured as follows. We provide a high-level overview of our system, implementing the proposed approach, in Section~\ref{sec:overview}. In Section~\ref{sec:recommendation}, we present and delve into the algorithm which generates cache-aware recommendations, as well as related implications and design choices. We evaluate the proposed system and algorithm in Section~\ref{sec:measurements}. In Section~\ref{sec:joint}, we further consider scenarios where the MEC cache is controlled by the operator, and we greedily optimize caching jointly with recommendations. After presenting related work in the field in Section~\ref{sec:related}, we conclude the paper.}


%\begin{itemize}

%\item However, proposed approaches require collaboration between network and content providers. E.g., in~\cite{}, ..., in~\cite{}. In practice, network providers are the ones who control the network and care most about the network performance (and capacity/congestion of the backhaul network), and content providers the ones who affect the traffic by controlling the recommendation system (at the end of the user/client) and the caching policy (at the end of the server; currently caching equipment in CDNs belongs to the content providers rather than the network providers). Moreover, content providers are not willing to share information about the user traffic (https is vastly used); in fact, this is one of the reasons that content providers currently control the caches (i.e., part of the infrastructure) themselves. Solutions for collaboration of content and network providers for caching require change of the architecture or protocols (e.g.,) \vassilis{@pavlos: 1-2 citations will suffice, but we need to show explicitly how we are better afterwards.} 

%\item We propose a solution that can bridge this gap, and be applied in today's networks (with existing infrastructure, protocols, etc.). Specifically, we propose that the network provider can leverage the recommendation system of the content provider to increase network efficiency (e.g., cache hit ratio in MEC\vassilis{What is MEC?}). We consider the case of YouTube, and propose a practical approach and design a system and algorithms that allow the network provider to exploit jointly recommendation and caching systems (even if they are both controlled by the content provider) to increase network efficiency. 

%\item We build an application (desktop and Android app) that (i) gets informed about the content cached in the edge/CDN/etc. cache, (ii) requests the related videos for a video from the YouTube API, (iii) builds a list of related and cached videos and recommends them to the user, (iv) delivers/streams the selected video from the YouTube servers or caches.

%\item The novelty of our approach is supported by the following observations: (i) No strong collaboration is required between the network and content provider. The network provider needs only information about the cached and related contents, which is currently available to it \vassilis{Are you sure that the net provider can easily find out the cached videos? We need to revisit the approach with the DNS queries probably, or propose a Youtube cache-provider interface.}. In particular, in the case of YouTube, our approach is immediately applicable. (ii) The recommendation algorithm exploits the recommendations system of the content service, searches through it to retrieve directly and indirectly related contents, and generates a list of related and cached contents to the user.

%\item Nevertheless, our approach can be applied to other online video/radio services, such as Netflix, Vimeo, Spotify, Pandora, where users consume sequentially content, and their traffic is highly affected by the recommendation systems. What is needed is an API that provides a list of related contents per requested content (or, even an ``offline search/crawling'' from the application that can discover content relations, extending thus the list of related contents directly provided by the content provider itself).

%\item Furthermore, our approach can be relevant to wireline networks and traditional CDNs as well: assuming a CDN cache usually located in the network of an ISP (or, MNO, etc.) or ``close'' to it (e.g., at an IXP infrastructure, which is closer to the ISP than the origin servers of the content provider), and an ISP that is aware of the content stored in the cache (which does not violate user privacy), we can apply the same approach and ``bias''\vassilis{we need to explain that what we do is not strongly biased, we try to do it without being too aggressive, breaking the original recommendation algorithm}  recommendations towards contents stored at the CDN cache, when, e.g., the network connecting the user to the origin servers is congested.

%\end{itemize}

==> JointCacheRec__BACKUP_07May2020.tex <==
In this section, we extend our study by considering the scenario where \ourAlgo and the caches are controlled by the same entity, e.g., the content provider. Network operator-controlled caching is the most commonly considered scenario in related work for MEC\pavlos{TODO add refs}; although in most of today's architectures the caches are actually controlled by the CP. 

In this scenario, the network operator can optimize caching decisions, thus further increasing the efficiency of \ourAlgo recommendations. Note that still there is no need for collaboration between the operator and the CP (e.g., possessing full knowledge of the RS), assumed in previous works~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching,giannakas-wowmom-2018}.

In the following, we first analytically formulate and study the problem of optimizing the caching policy, and propose an approximation algorithm with provable performance guarantees (\secref{sec:problem-algorithm}). We then evaluate the performance of this \textit{joint caching and recommendation} approach (\secref{sec:results-greedy}).

\subsection{Optimization Problem \&  Algorithm}
\label{sec:problem-algorithm}

Let a content catalog $\mathcal{V}$, $V=|\mathcal{V}|$, and a content popularity vector $\mathbf{q} = [q_{1}, ..., q_{V}]^{T}$. Let $\mathcal{L}(v)\subseteq \mathcal{V}$ be the set of contents that are explored by \ourAlgo (at \textit{line 1}) for a content $v\in\mathcal{V}$.%, and denote $\mathcal{L} = \bigcup_{v\in\mathcal{V}}\mathcal{L}(v)$.

For some set of cached contents $\mathcal{C}\subseteq\mathcal{V}$, and a content $v$, \ourAlgo returns a list of recommendations $\mathcal{R}(v)$ ($|\mathcal{R}(v)|=N$), in which at most $N$ contents $c\in \mathcal{C}\cap\mathcal{L}(v)$ appear at the top of the list. Therefore, CHR can be expressed as
\begin{equation}\label{eq:chr-generic}
CHR(\mathcal{C}) = \sum_{v\in\mathcal{V}}q_{v}\sum_{i=1}^{N(\mathcal{C},v)} p_{i}
\end{equation}
where $N(\mathcal{C},v) = \min\{|\mathcal{C}\cap\mathcal{L}(v)|, N\}$, and $p_{i}$ is the probability for a user to select the $i^{th}$ recommended content.% (as defined in \secref{sec:measurements}).

Then, the problem of optimizing the caching policy (to be jointly used with \ourAlgo), is formulated as follows:
\begin{equation}\label{optim-problem}
max_{\mathcal{C}} ~CHR(\mathcal{C})~~~~~s.t., |\mathcal{C}|\leq C
\end{equation}
where $C$ is the capacity of the --MEC-- cache.
% \begin{problem}
% \begin{align*}
% max_{\mathcal{C}} ~~~CHR(\mathcal{C})\\
% s.t., |\mathcal{C}|\leq C
% \end{align*}
% \end{problem}
We prove the following for the optimization problem of \eq{optim-problem}.
%We prove the following Lemma, whose proof is omitted due to space limitations.
\begin{mylemma}
The optimization problem of~\eq{optim-problem}: (i) is NP-hard, (ii) cannot be approximated within $1-\frac{1}{e}+o(1)$ in polynomial time, and (iii) has a monotone (non-decreasing) submodular objective function, and is subject to a cardinality constraint.
\end{mylemma}
\begin{proof}
Items (i) and (ii) of the above lemma, are proven by reduction to the \textit{maximum set coverage} problem, and we prove item (iii) using standard methods (see, e.g.,~\cite{femto,sermpezis-sch-globecom}). The detailed proof is omitted due to space limitations.
\pavlos{To add full proof}
\end{proof}

If we design a greedy algorithm that starts from an empty set of cached contents $\mathcal{C}_{g}=\emptyset$, and at each iteration it augments the set $\mathcal{C}_{g}$ (until $|\mathcal{C}_{g}|= C$) as follows:
\begin{equation}\label{eq:greedy-algo}
\mathcal{C}_{g}\leftarrow \mathcal{C}_{g}\cup \arg\max_{v\in\mathcal{V}} CHR(\mathcal{C}_{g}\cup\{v\}),
\end{equation}
then the properties stated in item (iii) satisfy that it holds~\cite{krause2012submodular}%for the solution yielded by a greedy algorithm $\mathcal{C}_{g}$ it holds~\cite{krause2012submodular} that:
\begin{equation}\label{eq:greedy-bound}
CHR(\mathcal{C}_{g}) \geq \left(1-\frac{1}{e}\right)\cdot CHR(\mathcal{C}^{*})
\end{equation}
where $\mathcal{C}^{*}$ the optimal solution of the problem of~\eq{optim-problem}. 

\textit{Remark}: While \eq{eq:greedy-bound} gives a lower bound for the performance of the greedy algorithm, in practice greedy algorithms have been shown to perform often very close to the optimal.\pavlos{add ref}

\subsection{Evaluation of Greedy Caching}\label{sec:results-greedy}

Calculating the CHR from \eq{eq:chr-generic} requires running a BFS (\ourAlgo, \textit{line 1}) and generating the lists $\mathcal{L}(v)$, for every content $v\in \mathcal{V}$. 


\myitem{Efficiency vs. scalability.} In practice, for scalability reasons, the most popular contents (i.e., with high $q_{i}$) can be considered by the greedy algorithm in the calculation of the objective function \eq{eq:chr-generic}, since those contribute more to the objective function. \blue{To demonstrate the involved trade-offs between scalability and performance, we consider two scenarios with synthetic content catalogs of size $|\mathcal{V}|$=1000 and $|\mathcal{V}|$=10000 (where content popularity $q_{i}$ follows a Zipf(a=1) distribution, and each content is related on average with $10$ other contents), and calculate the CHR achieved by \ourAlgo (N=10, $D_{BFS}$=2, $W_{BFS}$=5) when the greedy algorithm considers only a fraction $\mathcal{V}^{'}$ of the entire catalog, $\mathcal{V}^{'}\subseteq \mathcal{V}$, and a cache of size $C$=10. Table~\ref{tab:cabaret-greedy-vs-most-popular} presents the achieved CHR, normalized over the maximum CHR achieved when considering the entire catalog $\mathcal{V}$. We can see that even considering very small fractions of the content catalog in the caching decisions, can still achieve significant performance, while considering a 10\% of the content catalog can already achieve 90\% and 86\% of the maximum performance in the case of $|\mathcal{V}|$=1000 and $|\mathcal{V}|$=10000, respectively. This indicates that \ourAlgo-like approaches can be an efficient and scalable in real systems with very large content catalogs.}

%\pavlos{@Savvas: Add a plot for this scenario: Do a random content catalogue with K=1000 or 10000 contents with Zipf popularities (a=1), and a content matrix where each content is connected/related randomly with 10 or 20 other contents. Start considering in Eq.(1) only the q of the top x contents and run the greedy algorithm with C=10 or 50, let the sum of the popularities of the contents that are selected to be cached is y. Plot x vs y.}

\begin{table}[h]
\centering
\caption{\blue{CHR under caching with the greedy algorithm considering only a fraction of the most popular contents of the catalog, $i\in \mathcal{V}^{'}\subset \mathcal{V}$; values are normalized over the maximum achievable performance.}}
\label{tab:cabaret-greedy-vs-most-popular}
\begin{tabular}{cl|cccc}
\multicolumn{2}{c|}{fraction of the catalog $\frac{|\mathcal{V}^{'}|}{|\mathcal{V}|}$ }
    & 0.1\% & 1\% & 5\% & 10\%  \\
\hline
\multirow{2}{*}{$\frac{CHR(\mathcal{V}^{'})}{CHR(\mathcal{V})}$ }
& $|\mathcal{V}|=1000$
    & 0.72 & 0.74 & 0.89 & 0.90\\
& $|\mathcal{V}|=10000$            
    &  0.40 & 0.54  & 0.82  & 0.86 
\end{tabular}
\end{table}

%However, 
\blue{The reason that the greedy algorithm remains efficient even with this simplification, is that }%
any video in the catalog is still candidate to be cached, e.g., a video with low $q_{i}$ can bring a large increase in the CHR through its association with many popular contents. In fact, in our experiments, for the calculation of \eq{eq:chr-generic}, we consider only the 50 most popular videos, for which we set $q_{i} = \frac{1}{50}$. Nevertheless, in the different scenarios we tested, only 10\% to 30\% of the cached videos (selected by the greedy algorithm) were also in the top 50 most popular.%However, for the performance evaluation of CHR, we consider all involved contents, similarly to \secref{sec:results-single}. 

\myitem{Greedy vs. Top caching.} In Fig.~\ref{fig:chr-vs-c-greedy}, we compare the achieved CHR for ``Front Page'' video demand, when the cache is populated according to the greedy algorithm of \eq{eq:greedy-algo} (\textit{Greedy Caching}) and with the top most popular videos (\textit{Top Caching}). \textit{Greedy caching} always outperforms \textit{top caching}, with an increase in the CHR of around a factor of 2 for uniform video selection (for the Zipf($a$=1) scenarios we tested, the CHR values are even higher, and the relative performance is 1.5 times higher). This clearly demonstrates that the gains from joint recommendation and caching~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching}, are applicable even in simple practical scenarios (e.g., \ourAlgo \& greedy caching). Finally, while \textit{greedy caching} increases the CHR even with regular YouTube recommendations, the CHR is still less than $50\%$ of the \ourAlgo case with \textit{top caching}. This further stresses the benefits from \ourAlgo's cache-aware recommendations. 



\begin{figure}\centering
\centering
\subfigure[ ``Front Page'' video demand]{
\includegraphics[width=0.47\linewidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_uniform.eps}\label{fig:chr-vs-c-greedy}}
\subfigure[``Search Bar'' video demand]{
\includegraphics[width=0.47\linewidth]{./figuresSavvas/googleTrends/cacheSizeSearchZipf1GR.eps}\label{fig:greedyCachingZipf1GR}}
\caption{CHR vs. \# cached contents with \ourAlgo parameters $W_{BFS}$=50 and $D_{BFS}$=2, and video demand (a) ``Front Page'' video demand with $p_{i}\sim$\textit{uniform}, and (b) ``Search Bar'' video demand with  $p_{i}\sim$\textit{Zipf(a=1)} %GR region
.}
\end{figure}

\blue{Similar findings can be seen in Fig.~\ref{fig:greedyCachingZipf1GR} for scenarios with ``Search Bar'' video demand. A difference is that in these scenarios the CHR under YouTube recommendations with \textit{greedy caching} is comparable to \ourAlgo recommendations with \textit{top caching}, which indicates that similar performance can be achieved by carefully selecting either only the recommendations (\ourAlgo+ \textit{top caching}) or only the caching (YouTube + \textit{greedy caching}). However, when combining both (\ourAlgo + \textit{greedy caching}), increases more than two times the CHR.}


%%%COMMENTED OUT IN THE SHORT MEASUREMENTS VERSION
% \begin{figure}\centering
% \subfigure[uniform]{\includegraphics[width=0.47\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_uniform.eps}}
% \subfigure[Zipf($a$=1)]{\includegraphics[width=0.47\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_Zipf1.eps}}
% \vspace{-1\baselineskip}
% \caption{CHR vs. \# cached contents, for (a) \textit{uniform} and (b) \textit{Zipf($a$=1)} distribution of $p_{i}$ ($W_{BFS}$=50, $D_{BFS}$=2).}
% \label{fig:chr-vs-c-greedy}
% \end{figure}










% \begin{figure}\centering
% \begin{minipage}[t]{0.47\linewidth}
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_uniform.eps}
% \caption{\blue{CHR vs. C for $p_{i}\sim$\textit{uniform} ($N$=20, $W_{BFS}$=50, $D_{BFS}$=2).}\red{add pointer}}
% \label{fig:chr-vs-BFS-sequential}
% \end{minipage}
% %
% \hspace{0.03\linewidth}
% %
% \begin{minipage}[t]{0.47\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_Zipf1.eps}
% \caption{\blue{CHR vs. C for $p_{i}$ $\sim$\textit{Zipf($a$=1)} ($N$=20, $W_{BFS}$=50, $D_{BFS}$=2).}\red{add pointer}}
% \end{minipage}
% \end{figure}

==> JointCacheRec__BACKUP_31Mar18.tex <==
In this section, we extend our study by considering the scenario where \ourAlgo and the caches are controlled by the same entity, e.g., the network operator. Network operator-controlled caching is the most commonly considered scenario in related work for MEC; although in most of today's architectures the caches are actually controlled by the CP. 

In this scenario, the network operator can optimize caching decisions, thus further increasing the efficiency of \ourAlgo recommendations. Note that still there is no need for collaboration between the operator and the CP (e.g., possessing full knowledge of the RS), assumed in previous works~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching,giannakas-wowmom-2018}.

In the following, we first analytically formulate and study the problem of optimizing the caching policy, and propose an approximation algorithm with provable performance guarantees (\secref{sec:problem-algorithm}). We then evaluate the performance of this \textit{joint caching and recommendation} approach (\secref{sec:results-greedy}).

\subsection{Optimization Problem \&  Algorithm}
\label{sec:problem-algorithm}

Let a content catalog $\mathcal{V}$, $V=|\mathcal{V}|$, and a content popularity distribution $\mathbf{q} = [q_{1}, ..., q_{V}]^{T}$. Let $\mathcal{L}(v)\subseteq \mathcal{V}$ be the set of contents that are explored by \ourAlgo (at \textit{line 1}) for a content $v\in\mathcal{V}$, and denote $\mathcal{L} = \bigcup_{v\in\mathcal{V}}\mathcal{L}(v)$.

For some set of cached contents $\mathcal{C}\subseteq\mathcal{V}$, and a content $v$, \ourAlgo returns a list of recommendations $\mathcal{R}(v)$ ($|\mathcal{R}(v)|=N$), in which at most $N$ contents $c\in \mathcal{C}\cap\mathcal{L}(v)$ appear in the top of the list. Therefore, CHR can be expressed as
\begin{equation}\label{eq:chr-generic}
CHR(\mathcal{C}) = \sum_{v\in\mathcal{V}}q_{v}\sum_{i=1}^{N(\mathcal{C},v)} p_{i}
\end{equation}
where $N(\mathcal{C},v) = \min\{|\mathcal{C}\cap\mathcal{L}(v)|, N\}$, and $p_{i}$ is the probability for a user to select the $i^{th}$ recommended content.% (as defined in \secref{sec:measurements}).

Then, the problem of optimizing the caching policy (to be jointly used with \ourAlgo), is formulated as follows:
\begin{equation}\label{optim-problem}
max_{\mathcal{C}} ~CHR(\mathcal{C})~~~~~s.t., |\mathcal{C}|\leq C
\end{equation}
where $C$ is the capacity of the --MEC-- cache.
% \begin{problem}
% \begin{align*}
% max_{\mathcal{C}} ~~~CHR(\mathcal{C})\\
% s.t., |\mathcal{C}|\leq C
% \end{align*}
% \end{problem}
We prove the following for the optimization (OPT) problem of \eq{optim-problem}.
%We prove the following Lemma, whose proof is omitted due to space limitations.
\begin{mylemma}
The OPT problem of~\eq{optim-problem}: (i) is NP-hard, (ii) cannot be approximated within $1-\frac{1}{e}+o(1)$ in polynomial time, and (iii) has a monotone (non-decreasing) submodular objective function, and is subject to a cardinality constraint.
\end{mylemma}
\begin{proof}
Items (i) and (ii) of the above lemma, are proven by reduction to the maximum set coverage problem, and we prove item (iii) using standard methods (see, e.g.,~\cite{femto,sermpezis-sch-globecom}). The detailed proof is omitted due to space limitations.
\end{proof}

If we design a greedy algorithm that starts from an empty set of cached contents $\mathcal{C}_{g}=\emptyset$, and at each iteration it augments the set $\mathcal{C}_{g}$ (until $|\mathcal{C}_{g}|= C$) as follows:
\begin{equation}\label{eq:greedy-algo}
\mathcal{C}_{g}\leftarrow \mathcal{C}_{g}\cup \arg\max_{v\in\mathcal{V}} CHR(\mathcal{C}_{g}\cup\{v\}),
\end{equation}
then the properties stated in item (iii) satisfy that it holds~\cite{krause2012submodular}%for the solution yielded by a greedy algorithm $\mathcal{C}_{g}$ it holds~\cite{krause2012submodular} that:
\begin{equation}\label{eq:greedy-bound}
CHR(\mathcal{C}_{g}) \geq \left(1-\frac{1}{e}\right)\cdot CHR(\mathcal{C}^{*})
\end{equation}
where $\mathcal{C}^{*}$ the optimal solution of the problem of~\eq{optim-problem}. 

\textit{Remark}: While \eq{eq:greedy-bound} gives a lower bound for the performance of the greedy algorithm, in practice greedy algorithms have been shown to perform often very close to the optimal.

\subsection{Evaluation of Greedy Caching}\label{sec:results-greedy}

Calculating the CHR from \eq{eq:chr-generic} requires running a BFS (\ourAlgo, \textit{line 1}), generating the lists $\mathcal{L}(v)$ for every content $v\in \mathcal{V}$. In practice, for scalability reasons, the most popular contents (i.e., with high $q_{i}$) can be considered by the greedy algorithm in the calculation of the objective function \eq{eq:chr-generic}, since those contribute more to the objective function. However, any video in the catalog is still candidate to be cached, e.g., a video with low $q_{i}$ can bring a large increase in the CHR through its association with many popular contents.

In fact, in our experiments, for the calculation of \eq{eq:chr-generic}, we consider only the 50 most popular videos, for which we set $q_{i} = \frac{1}{50}$. Nevertheless, in the different scenarios we tested, only 10\% to 30\% of the cached videos (selected by the greedy algorithm) were also in the top 50 most popular.%However, for the performance evaluation of CHR, we consider all involved contents, similarly to \secref{sec:results-single}. 

In Fig.~\ref{fig:chr-vs-c-greedy}, we compare the achieved CHR when the cache is populated according to the greedy algorithm of \eq{eq:greedy-algo} (\textit{Greedy Caching}), and with the top most popular videos (\textit{Top Caching}).%; as in previous sections).
~\textit{Greedy caching} always outperforms \textit{top caching}, with an increase in the CHR of around $2\times$ and $1.5\times$ in the uniform and Zipf($a$=1) scenarios, respectively. This clearly demonstrates that the gains from joint recommendation and caching~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching}, are applicable even in simple practical scenarios (e.g., \ourAlgo \& greedy caching). Finally, while \textit{greedy caching} increases the CHR even with regular YouTube recommendations, the CHR is still less than $50\%$ of the \ourAlgo case with \textit{top caching}. This further highlights the benefits from using \ourAlgo for cache-aware recommendations. 


\begin{figure}\centering
\subfigure[uniform]{\includegraphics[width=0.47\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_uniform.eps}}
\subfigure[Zipf($a$=1)]{\includegraphics[width=0.47\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_Zipf1.eps}}
\vspace{-1\baselineskip}
\caption{CHR vs. \# cached contents, for (a) \textit{uniform} and (b) \textit{Zipf($a$=1)} distribution of $p_{i}$ ($W_{BFS}$=50, $D_{BFS}$=2).}
\label{fig:chr-vs-c-greedy}
\end{figure}
% \begin{figure}\centering
% \begin{minipage}[t]{0.47\linewidth}
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_uniform.eps}
% \caption{\blue{CHR vs. C for $p_{i}\sim$\textit{uniform} ($N$=20, $W_{BFS}$=50, $D_{BFS}$=2).}\red{add pointer}}
% \label{fig:chr-vs-BFS-sequential}
% \end{minipage}
% %
% \hspace{0.03\linewidth}
% %
% \begin{minipage}[t]{0.47\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_C_greedy_caching_W50_D2_Zipf1.eps}
% \caption{\blue{CHR vs. C for $p_{i}$ $\sim$\textit{Zipf($a$=1)} ($N$=20, $W_{BFS}$=50, $D_{BFS}$=2).}\red{add pointer}}
% \end{minipage}
% \end{figure}

==> Measurements__BACKUP_31Mar18.tex <==
%In this section, w
We perform measurements and experiments over the YouTube service\footnote{Our experiments and use of the YouTube API conform to the YouTube terms of service \url{https://www.youtube.com/static?template=terms}.}, to investigate the performance (in terms of cache hit ratios) of our approach in MEC scenarios. The setup of the scenarios is presented in \secref{sec:experiments-setup}, and the results in~\secref{sec:results}.


\subsection{Setup}
\label{sec:experiments-setup}

%\subsection{The YouTube API}
\myitem{The YouTube API} provides a number of functions to retrieve information about videos, channels, user ratings, etc. In our measurements, we request %(a) the most popular videos in a region (max. 50), and (b) the list of related videos (max. 50) for a given video.
%
the following information:
\begin{itemize}
\item the most popular videos in a region (max. 50)%, e.g., \red{[@Savvas: is there any concise command we could add here?]}
\item the list of related videos (max. 50) for a given video
\end{itemize}
\red{\textit{Remark}: In the remainder, we present results collected during March 2017, for the region of Greece (GR). While our insights hold also for other regions we tested, we briefly state results for the region of United States (US) for completeness.}
% %\red{[Write how much quota we have and to how many requests for related videos they correspond]}

%\subsection{Measurement Scenarios}
%We consider the following experimental scenario.
%over which we conduct the measurements and experiments, 
%as follows.% The setup of the scenarios is as follows.

\myitem{Caching.} We assume a MEC cache storing the most popular videos in a region. We populate the list of cached contents with the top $C$ %(C=$|\mathcal{C}|$)
video IDs returned from the YouTube API.

\myitem{Recommendations.} We consider two classes of scenarios with (i) YouTube and (ii) \ourAlgo recommendations. In both cases, when a user enters the UI, the $50$ most popular videos in her region are recommended to her (as in YouTube's front page). Upon watching a video $v$, a list of $N=20$ videos is recommended to the user; the list is (i) composed of the top $N$ directly related videos returned from the YouTube API (YouTube scenarios), or (ii) generated by \ourAlgo with parameters $N$, $W_{BFS}$ and $D_{BFS}$ (\ourAlgo scenarios).
%the list of $N$ contents generated by \ourAlgo is recommended to her.% with parameters $\{v,N,W_{BFS},D_{BFS}\}$.

\myitem{Video Demand.} In each experiment, we assume a user that enters the UI and watches one of the initially recommended (i.e., $50$ most popular) videos at random. Then, the system recommends a list of $N$ videos ($r_{1},r_{2},...,r_{N}$), and the user selects with probability $p_{i}$ to watch $r_{i}$ next. We set $p_{i}$ to depend on the order of appearance --and not the content--
and consider \textit{uniform} ($p_{i}=\frac{1}{N}$) and \textit{Zipf} ($p_{i}\sim\frac{1}{i^{\alpha}}$) scenarios; the higher the exponent $\alpha$ of the Zipf distribution, the more preference is given by the user to the top recommendations (user preference to top recommendations has been observed in YouTube traffic~\cite{cache-centric-video-recommendation}).
%We simulate \red{$M$} experiments, where a user enters the UI and watches randomly one of the initially recommended (i.e., most popular) videos%; let video $v_{0}$

%We simulate $M$ experiments. In each experiment, a user enters the application and selects randomly one of the recommended (i.e., most popular) videos; let video $v_{0}$. The application recommends to her a list of $N$ contents ($r_{1},r_{2},...,r_{N}$). The users selects with probability $p_{i}$ to request next the $r_{i}$ content, where we assume that the probability $p_{i}$ depends on the order of appearance and not on the video IDs. \vassilis{Can we justify this with related work?}

\subsection{Results}\label{sec:results}
\subsubsection{Single Request}\label{sec:results-single}~\\
We first consider scenarios of single requests (similarly to~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching}). In each experiment $i$ ($i=1,...,M$) a user watches one of the top popular videos, let $v_{1}(i)$, and then follows a recommendation and watches a video $v_{2}(i)$. We measure the Cache Hit Ratio (CHR), which we define as the fraction of the \textit{second requests} of a user that are for a cached video (since the first request is always for a cached --top popular-- one):
%. Let the second request of an experiment $i$ be for a content $v_{2}(i)$, then CHR is given by 
\begin{equation*}
%\mbox{$
\textstyle
CHR = \frac{1}{M}\cdot \sum_{i=1}^{M} \mathbb{I}_{v_{2}(i)\in \mathcal{C}}
%$},
\end{equation*}
where $\mathbb{I}_{v_{2}(i)\in \mathcal{C}} =1$ if $v_{2}(i)\in \mathcal{C}$ and $0$ otherwise, and $M$ the number of experiments\footnote{We considered all possible experiments on the collected dataset.}.
% $
% \mathbb{I}_{v_{1}(i)\in C} = \left\{ 
% \begin{tabular}{ll}
% 1&, if $v_{1}(i)\in C$\\
% 0&, otherwise
% \end{tabular}
% \right.
% $%\end{equation*}

%\subsection{Results}
\myitem{CHR vs. BFS parameters.} Fig.~\ref{fig:chr-vs-bfs-param} shows the CHR achieved by \ourAlgo under various parameters, along with the CHR under regular YouTube recommendations, when caching all the most popular videos ($|\mathcal{C}|$=50). The efficiency of caching significantly increases with \ourAlgo, even when only directly related contents are recommended ($D_{BFS}$=1), i.e., \textit{without loss in recommendation quality}. Just reordering the list of YouTube recommendations (as suggested in~\cite{cache-centric-video-recommendation}), brings gains when $p_{i}$ is not uniformly distributed. However, the added gains by our approach are significantly higher. As expected, the CHR increases for larger $W_{BFS}$ and/or $D_{BFS}$; e.g., \ourAlgo for $W_{BFS}$=50 and $D_{BFS}$=2, achieves $\times8-\times10$ higher CHR than regular YouTube recommendations. Also, the CHR increases for more skewed $p_{i}$ distributions, since top recommendations are preferred and \ourAlgo places cached contents in the top of the recommendation list.

In Fig.~\ref{fig:chr-vs-W} we observe that, when higher preference is given to top recommendations, increasing the $W_{BFS}$ can increase CHR even with $D_{BFS}$=1. However, for uniform selection, significant gains cannot be brought only by increasing $W_{BFS}$. This indicates that, in such cases, considering also indirectly related contents (i.e., $D_{BFS}>1$, as \ourAlgo does), is required to yield a non-negligible increase in CHR (cf. Fig.~\ref{fig:chr-vs-bfs-param}). 


\begin{figure}\centering
\begin{minipage}[t]{0.46\linewidth}
\includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_probability.eps}
\caption{CHR under different BFS parameters % (for N=20)
.}
\label{fig:chr-vs-bfs-param}
\end{minipage}
%
\hspace{0.03\linewidth}
%
\begin{minipage}[t]{0.47\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_W_N20_D1.eps}
\caption{CHR vs. $W_{BFS}$ \\($D_{BFS}$=1)%(for N=20 and $D_{BFS}$=1)
.}
\label{fig:chr-vs-W}
\end{minipage}
\end{figure}



\myitem{CHR vs. number of cached videos.} We further consider scenarios with varying number of cached contents $C = |\mathcal{C}|$. In each scenario, we assume that the $C$ most popular contents are cached. Fig.~\ref{fig:chr-vs-C-d2} %Figures~\ref{fig:chr-vs-C-d1} and~\ref{fig:chr-vs-C-d2} show
shows the CHR achieved by \ourAlgo, in comparison to scenarios under regular YouTube recommendations. The results are consistent for all considered values of $C$: the CHR under \ourAlgo is significantly higher than in the YouTube case. Moreover, even when caching a small subset of the most popular videos, \ourAlgo brings significant gains. E.g., by caching $C=10$ out of the $50$ top related contents \ourAlgo increases the CHR from $2\%$ and $3.2\%$ to $17\%$ and $50\%$, for the uniform and Zipf($\alpha$=1) scenarios, respectively.


\begin{figure}\centering
\begin{minipage}[t]{0.47\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_cache_size_W50_D2.eps}
\caption{CHR vs.\\ \#~cached contents $C$\\ ($W_{BFS}$=50, $D_{BFS}$=2).}
\label{fig:chr-vs-C-d2}
\end{minipage}
%
\hspace{0.03\linewidth}
%
\begin{minipage}[t]{0.47\linewidth}
\includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_K_sequential_requests_W20_D2_C20.eps}
\caption{CHR vs. \#~requests in sequence $K$ ($C$=20, $W_{BFS}$=20, $D_{BFS}$=2). \textit{Note}: y-axis up to 40\%.}
\label{fig:chr-vs-K-sequential}
\end{minipage}
\end{figure}

%%%% CHR vs. C: depth 1 and 2, in one figure
% \begin{figure}\centering
% \subfigure[$D_{BFS}$=1]{\includegraphics[width=0.47\columnwidth]{./figures/fig_CHR_vs_cache_size_W50_D1.eps}\label{fig:chr-vs-C-d1}}
% \subfigure[$D_{BFS}$=2]{\includegraphics[width=0.47\columnwidth]{./figures/fig_CHR_vs_cache_size_W50_D2.eps}\label{fig:chr-vs-C-d2}}
% \vspace{-\baselineskip}\caption{CHR vs. number of cached contents $C$ for scenarios with %$N$=20, 
% $W_{BFS}$=50, and (a) $D_{BFS}$=1 or (b) $D_{BFS}$=2.}
% \label{fig:chr-vs-C}
% \end{figure}

%%%% CHR vs. C: depth 1 and 2, in two figures
% \begin{figure}\centering
% \begin{minipage}[t]{0.47\linewidth}
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_cache_size_W50_D1.eps}
% \caption{\blue{CHR vs. C ($N$=20, $W_{BFS}$=50, $D_{BFS}$=1).}}
% \label{fig:chr-vs-C-d1}
% \end{minipage}
% %
% \hspace{0.03\linewidth}
% %
% \begin{minipage}[t]{0.47\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_cache_size_W50_D2.eps}
% \caption{\blue{CHR vs. C ($N$=20, $W_{BFS}$=50, $D_{BFS}$=2).}}
% \label{fig:chr-vs-C-d2}
% \end{minipage}
% \end{figure}




\subsubsection{Sequential Requests}~\\
We now test the performance of our approach in scenarios where users enter the system and watch a sequence of $K$, $K>2$, videos (similarly to~\cite{giannakas-wowmom-2018}, and in contrast to the previous case, where they watch only two videos, i.e., $K=2$). At each step, the system recommends a list of videos to the user by applying \ourAlgo on the currently watched video. We denote as $v_{k}(i)$ the $k^{th}$ video requested/watched by a user at experiment $i$. We measure the CHR, which is now defined as
\begin{equation*}
%\mbox{$
\textstyle
CHR = \frac{1}{M}\cdot \sum_{i=1}^{M} \sum_{k=2}^{K} \mathbb{I}_{v_{k}(i)\in \mathcal{C}}
%$},
\end{equation*}
where $\mathbb{I}_{v_{k}(i)\in \mathcal{C}} =1$ if $v_{k}(i)\in \mathcal{C}$ and $0$ otherwise, over $M=100$ experiments per scenario.


While moving ``farther'' from the initial requested video (which belongs to the list of most popular and cached videos) through a sequence of requests, we expect the CHR to decrease, due to lower similarity of the requested and cached videos. However, as Fig.~\ref{fig:chr-vs-K-sequential} shows, the decrease in the CHR (under \ourAlgo recommendations) is not large. The CHR remains close to the case of single requests (i.e., for $K$=2 in the x-axis), indicating that our approach performs well even when we are several steps far from the cached videos. In fact, caching more than the top most popular videos appearing on the front page, would further reduce the CHR decrease.

%%%% CHR vs. sequential requests:in two figures
% \begin{figure}\centering
% \begin{minipage}[t]{0.47\linewidth}
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_K_sequential_requests_W20_D2_C20.eps}
% \caption{\blue{CHR vs. number of sequential requests $K$ for $C$=20\\ ($N$=20, $W_{BFS}$=20, $D_{BFS}$=2).}\red{ Note: scale of y-axis up to 40\%}}
% \label{fig:chr-vs-K-sequential}
% \end{minipage}
% %
% \hspace{0.03\linewidth}
% %
% \begin{minipage}[t]{0.47\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{./figures/fig_CHR_vs_C_sequential_requests__K5_W20_D2.eps}
% \caption{\blue{CHR vs. C for $K$=5 sequential requests  ($N$=20, $W_{BFS}$=20, $D_{BFS}$=2).}\red{ Note: scale of y-axis up to 40\%}}
% \label{fig:chr-vs-C-sequential}
% \end{minipage}
% \end{figure}


==> RecAlgo__BACKUP_20Apr2020.tex <==
\red{
\begin{itemize}
    \item realistic evaluation - no required data
    \item lowers the barrier for techno-ecomonic feasibility of the paradigm. The same approach could be applied in practice, even in cases where it is not the same entity that controls both network and RS; there are no strong requirements for knowledge exchange
    \item Even in the case of the same entity, it is an alternative approach compared to what has been proposed now. Allows a modular system architecture, that minimized interdependencies between network/RS compoments. This can lead to more robust architecture, increased privacy, but more importantly to higher scalability (e.g., most previous approaches require the knowledge of the entire catalog, which is huge in practice) - except Livia (others?); while this comes at a cost of performance, we demonstrate in section \ref{} that a good trade-off between performance and scalabitity is feasible in practice. 
\end{itemize}
}


%\subsection{Design and Rationale}\label{sec:design-rationale}

%\begin{itemize}
%\item The works in~\cite{} propose to explore related contents, and select the most related contents (with preference to those that are cached) to recommend to the user. However, this action requires the system to be aware of the ``content relations'' (e.g., the similarity score of contents, the user preferences, past data and/or statistics for the user, content trends, etc.). This information is owned by the service provider, who is highly unlikely to disclose it to third parties, due to privacy and economic reasons (usually this data is a main source of income for the content providers, e.g., for advertising). Hence, such approaches would require to be controlled by the content provider. On the contrary we propose the network provider to indirectly retrieve this information, i.e., related videos, from the recommendation system of the content service, i.e., the recommendations that the service would do to a user. To this end, we exploit the YouTube API, which allows to obtain information about related videos.
%\item The recommendation algorithm: (i) requests the maximum number of the contents related to the YouTube video that is currently consumed by the user; (ii) it starts a BFS for each of these videos, i.e., requests the related videos for each of the contents in the initial list of videos (the BFS can continue deeper as seen in Fig.~\ref{}). It builds an ordered list with the related videos, sorting videos by the order they appear in the BFS depth, and the order they are provided for each depth of the BFS. Selects in this list the videos that are also cached (if any), and recommends to the user the top \red{N} videos. If needed, i.e., less than \red{N} cached videos appear in the list of related videos, then it recommends the remaining videos from the initial list of related videos.
%\end{itemize}

In existing approaches, e.g.,~\cite{sermpezis-sch-globecom,chatzieleftheriou2017caching,giannakas-wowmom-2018}\red{[TODO: add more refs, rephrase next sentence]}, the ``most related'' contents that are also cached, are recommended to users. 
However, this requires the system to be aware of the \textit{content relations} (e.g., similarity scores, user preferences/history, trending videos), i.e., information owned by the content provider. Such data are unlikely to be disclosed to third parties, due to privacy and/or economic reasons (e.g.,~advertising). %As a result, approaches would require to be controlled by the content provider. 
% (usually this data is a main source of income for the content providers, e.g., for advertising)

In our approach, the system leverages information about content relations that is made publicly available by the RS of the content service (i.e., YouTube in this paper). In particular, when a user watches a video $v$, the system requests from the YouTube API a list of video IDs $\mathcal{L}$ related to $v$, i.e., the videos that YouTube would recommend to the user. Then it requests the related video IDs for every video in $\mathcal{L}$ and adds them in the end of $\mathcal{L}$, and so on, in a Breadth-First Search (BFS) manner. In the end of the process, the list $\mathcal{L}$ contains IDs of videos directly and indirectly related to $v$; of these videos, the top $N$ that are cached and/or highly related to $v$ are finally recommended to the user. The list $\mathcal{L}$ is (i) much larger than the list of videos recommended by YouTube, and thus it is more probable to contain cached videos that are related to $v$, and (ii) built based on video relations provided by YouTube itself, which satisfies a high quality of recommendations.

%In fact, using the YouTube recommendations ensures strong relations between videos that are directly related to $v$ (i.e., BFS at depth 1). Moreover, while the YouTube RS finds hundreds of videos highly related to $v$, only a subset of them are recommended to the user~\cite{covington2016deep}. The rationale behind our recommendation algorithm is to explore the related videos that are not communicated to the user. To this end, based on the fact that related videos are similar and have high probability of sharing recommendations (i.e., if video $a$ is related to $b$, and $b$ to $c$, then it is probable that $c$ relates to $a$), the algorithm tries to infer these latent video relations through BFS. Hence, videos found by BFS in depths $>1$ are also (indirectly) related to $v$ and probably good recommendations as well.

We detail our recommendation algorithm (\ourAlgo) in \secref{sec:detailed-algo}, and discuss the related design implications in \secref{sec:tune-algo}.

\begin{figure}
\centering
\includegraphics[width=1\linewidth,height=0.6\linewidth]{./figures/Scheme_2_new.eps}
\caption{CABaRet: example with $D_{BFS}=2$, $W_{BFS}=3$, $N=6$. Cached videos are denoted with black color.}
\label{fig:rec-algo}
\end{figure}


\subsection{The Recommendation Algorithm}\label{sec:detailed-algo}

\myitem{Input.} The recommendation algorithm receives as input:
\begin{itemize}[leftmargin=*]
\item $v$: the video ID (or URL) which is currently watched
\item $N$: the number of videos to be recommended
\item $\mathcal{C}$: the list with the IDs of the cached videos
\item $D_{BFS}$: the depth to which the BFS proceeds
\item $W_{BFS}$: the number of related videos that are requested \textit{per content} from the YouTube API (i.e., the ``width'' of BFS)
\end{itemize}

\myitem{Output.} The recommendation algorithm returns as output:
\begin{itemize}[leftmargin=*]
\item $\mathcal{R}$: ordered list of $N$ video IDs to be recommended.
\end{itemize}
%\vspace{\baselineskip}
\myitem{Workflow.} \ourAlgo searches for videos related to video $v$ in a BFS manner as follows (\textit{line 1} in Algorithm~\ref{alg:recommendation}). Initially, it requests the $W_{BFS}$ videos related to $v$, and adds them to a list $\mathcal{L}$ in the order they are returned from the YouTube API. For each video in $\mathcal{L}$, it further requests $W_{BFS}$ related videos, as shown in Fig.~\ref{fig:rec-algo}, and adds them in the end of $\mathcal{L}$. It proceeds similarly for the newly added videos, until the depth $D_{BFS}$ is reached; e.g., if $D_{BFS}=2$, then $\mathcal{L}$ contains $W_{BFS}$ video IDs related to $v$, and $W_{BFS}\cdot W_{BFS}$ video IDs related to the related videos~of~$v$.

Then, \ourAlgo searches for video IDs in $\mathcal{L}$ that are also included in the list of cached videos $\mathcal{C}$ %i.e., $c \in \mathcal{L} \cap \mathcal{C}$)
and adds them to the list of video IDs to be recommended $\mathcal{R}$, until all IDs in $\mathcal{L}$ are explored or the list $\mathcal{R}$ contains $N$ video IDs, whichever comes first (\textit{lines 4--9}).
%Then, in \red{lines 4--9}, it searches in the ordered list $\mathcal{L}$ (starting from the first element in the list) for video IDs that are also included in the list of cached videos $\mathcal{C}$. When a video $c \in \mathcal{L} \cap \mathcal{C}$ is found, it is added in the list of video IDs to be recommended $\mathcal{R}$. This continues until all the IDs in $\mathcal{L}$ are explored or the list $\mathcal{R}$ contains $N$ video IDs, whichever comes first. 
If after this step, $\mathcal{R}$ contains less than $N$ video IDs, $N-|\mathcal{R}|$ video IDs from the head of the list $\mathcal{L}$ are added to $\mathcal{R}$; these IDs correspond to the top $N-|\mathcal{R}|$ non-cached videos that are directly related to video $v$ (\textit{lines 10--15}).
%After this step, in \red{lines 10--15}, if $\mathcal{R}$ contains less than $N$ video IDs, $|\mathcal{R}|-N$ video IDs from the head of the list $\mathcal{L}$ are added to $\mathcal{R}$; these IDs correspond to the the top $|\mathcal{R}|-N$ non-cached videos that are directly related to video $v$.

%Finally, the ordered list $\mathcal{R}$ of the IDs of the videos to be recommended is returned (\red{line 16}).

\begin{algorithm}
%\begin{small}
\begin{algorithmic}[1]
\caption{\\~\textit{CABaRet}: Cache-Aware \& BFS-related  Recommendations}\label{alg:recommendation}
\Statex {$Input: v, N, \mathcal{C}, D_{BFS}, W_{BFS}$} 
%\Statex \Comment $v$: initial video request
%\Statex \Comment $N$: number of contents to recommend
%\Statex \Comment $\mathcal{C}$: set of cached contents
%\Statex \Comment $D_{BFS}$ depth of BFS
%\Statex \Comment $W_{BFS}$ width of BFS
\State $\mathcal{L}\gets BFS(v,D_{BFS},W_{BFS})$ \Comment ordered set of video IDs
\State $\mathcal{R}\gets \emptyset$ \Comment ordered set of video IDs to be recommended
\State $i\gets 1$
\For {$c\in \mathcal{L}$}
	\If {$i\leq N$ and $c\in \mathcal{C}$}
		\State $\mathcal{R}.{append}(c)$
		\State $i\gets i+1$
	\EndIf
\EndFor
\For {$c\in \mathcal{L}\setminus \mathcal{R}$}
	\If {$i\leq N$}
    	\State $\mathcal{R}.{append}(c)$
		\State $i\gets i+1$
    \EndIf
\EndFor

%\While {$i\leq N$ and $\mathcal{L}\setminus \mathcal{R} \neq \emptyset$}
%	\For {$c\in \mathcal{L}\setminus \mathcal{R}$}
%		\State $\mathcal{R}.{append}(c)$
%		\State $i\gets i+1$
%	\EndFor
%\EndWhile
\State $return~~\mathcal{R}$
\end{algorithmic}
%\end{small}
\end{algorithm}


\subsection{Implications and Design Choices}\label{sec:tune-algo}
%\subsection{Tuning the Recommendation Algorithm}\label{sec:tune-algo}

\myitem{High-quality recommendations.} Using the YouTube recommendations ensures strong relations between videos that are directly related to $v$ (i.e., BFS at depth 1). Moreover, while the YouTube RS finds hundreds of videos highly related to $v$, only a subset of them are recommended to the user~\cite{covington2016deep}. The rationale behind \ourAlgo is to explore the related videos that are not communicated to the user. To this end, based on the fact that related videos are similar and have high probability of sharing recommendations (i.e., if video $a$ is related to $b$, and $b$ to $c$, then it is probable that $c$ relates to $a$)\red{[TODO: add ref to item-item similarity, check related work for this type of recommendation in YouTube]}, \ourAlgo tries to infer these latent video relations through BFS. Hence, videos found by BFS in depths $>1$ are also (indirectly) related to $v$ and probably good recommendations as well.

To further support the above claim, we collect and analyze datasets of related YouTube videos. Specifically, we consider the set of most popular  videos, let $\mathcal{P}$, in a region, and for each $v\in\mathcal{P}$ we perform BFS by requesting the list of related videos (similarly to \textit{line 1} in \ourAlgo). We use as parameters $W_{BFS}=\{10,20,50\}$ and $D_{BFS}=2$, i.e., considering the directly related videos (depth 1) and indirectly related videos with depth 2. We denote as $\mathcal{R}_{1}(v)$ and $\mathcal{R}_{2}(v)$, the set of videos found at the first and second depth of the BFS, respectively. We calculate the fraction of the videos in $\mathcal{R}_{1}(v)$ that are also contained in $\mathcal{R}_{2}(v)$, i.e., $I(v) = \frac{| \mathcal{R}_{1}(v)  \cap \mathcal{R}_{2}(v)|}{|\mathcal{R}_{1}(v)|}$. High values of $I(v)$ indicate a strong similarity of the initial content $v$ with the set of indirectly related contents at depth 2. 


Table~\ref{table:I-v} shows the median values of $I(v)$, over the $|\mathcal{P}|=50$ most popular contents in the region of Greece (GR), for different BFS widths. As it can be seen, $I(v)$ is very high for most of the initial videos $v$. For larger values of $W_{BFS}$, $I(v)$ increases, and when we fully exploit the YouTube API capability, i.e., for $W_{BFS}$=50, which is the maximum number of related videos returned by the YouTube API, the median value of $I(v)$ becomes larger than $0.9$. Finally, we measured the $I(v)$ in other regions as well, and observed that even in large (size/population) regions, the $I(v)$ values remain high, e.g., in the United States (US) region, $I(v)$=0.8 for $W_{BFS}$=50.
%Finally, we measured the $I(v)$ in other regions as well. While larger (size/population) regions have on average lower $I(v)$ values, there are always many common directly and indirectly related videos, e.g., in the large region of United States (US) $I(v)=0.8$ for $W_{BFS}=50$.


%Table~\ref{table:I-v} shows the median values of $I(v)$, over the $|\mathcal{P}|=50$ most popular contents in the region of Greece (GR), for different BFS widths. As it can be seen, the intersection of directly ($\mathcal{R}_{1}(v)$) and indirectly ($\mathcal{R}_{2}(v)$) related videos, is very high for most of the initial videos $v$. For larger values of $W_{BFS}$, the intersection increases; when we fully exploit the YouTube API capability, i.e., for $W_{BFS}=50$, which is the maximum number of related videos returned by the YouTube API, the median value of $I(v)$ becomes larger than $0.9$. Finally, we measured the $I(v)$ in other regions as well. While larger (size/population) regions have on average lower $I(v)$ values, there are always many common directly and indirectly related videos, e.g., in the region of United States (US) the median $I(v)$ is $0.6$ for $W_{BFS}=50$.


% Fig.~\ref{fig:intersection-vs-W} shows the distribution (boxplots) of $I(v)$, over the $|\mathcal{P}|=50$ most popular contents in a region, for different BFS widths (x-axis). As it can be seen, the intersection of directly ($\mathcal{R}_{1}(v)$) and indirectly ($\mathcal{R}_{2}(v)$) related videos, is very high for most of the initial videos $v$, under any case. For larger values of $W_{BFS}$, the intersection increases; when we fully exploit the YouTube API capability, i.e., for $W_{BFS}=50$, which is the maximum number of related videos returned by the YouTube API, the median value of $I(v)$ becomes larger than $90\%$.}\pavlos{I think we should consider the sets at depth 1 always with W=50, and plot vs. the width of the depth 2 steps only.} \vassilis{Is this fixed? Or it still applies?}
\begin{table}[h]
\centering
\caption{$I(v)$ vs. $W_{BFS}$ for the region of GR% (left table), and $I(v)$ vs. region for $W_{BFS}=50$ (right table)
.}
%\vspace{-\baselineskip}
\label{table:I-v}
\begin{tabular}{|cccc|%c|cccc|
}
\hline
{$W_{BFS}:$}	&{10}&{20}&{50}%&{}&{Region:}	&{GR} & {FR} & {US}
\\
{$I(v):$}	&0.70&0.85&0.92%&{}&{$I(v)$:}	&0.92 & 0.69 & 0.60
\\
\hline
\end{tabular}
\vspace{-\baselineskip}
\end{table}

% NO TIME for this comment, deactivating it
%\vassilis{Could we also check how frequently the top-X videos, that are downloaded in the cache, are changing content- or order-wise? What I do not know if whether the ``quality'' of the cache recommendations is deteriorating as long as we do not update it within certain frequency intervals. Meaning: maybe the CHR is fine at time t, but after an hour the results vary wildly. We need to check the stability of figures 5-8!}

%\vassilis{Update on comment above: the contents change significantly on a daily basis (most popular and their D1-related, so the cache needs to be refreshed daily (at least).}
%\pavlos{Check if the values of the quantity I(v) remain similar, despite the fact that the most popular change. This would show that our results are robust wrt to YouTube traffic differentiations.} \vassilis{Not able to address this due to lack of data. Study over time is moved in future work.}


% \begin{figure}\centering
% \begin{minipage}[t]{0.47\linewidth}
% \includegraphics[width=1\columnwidth]{./figures/fig_Intersection_D1andD2_vs_W.eps}
% \caption{\blue{Distribution of $I(v)$ values for different $W_{BFS}$.}}
% \label{fig:intersection-vs-W}
% \end{minipage}
% %
% \hspace{0.03\linewidth}
% %
% \begin{minipage}[t]{0.47\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{./figures/empty.eps}
% \caption{\pavlos{Here we could have plots for 3-4 different regions, for $W_{BFS}=50$} \vassilis{also we need to refer to it somewhere in the text}}
% \label{fig:}
% \end{minipage}
% \end{figure}

\myitem{Tuning \ourAlgo.} 
The parameters $D_{BFS}, W_{BFS}$ can be tuned to achieve a desired performance, e.g., in terms of probability of recommending a cached or highly related video.
%
For large $D_{BFS}$, the similarity between $v$ and the videos \textit{at the end of the list} $\mathcal{L}$ is expected to weaken, while for small $D_{BFS}$ the list $\mathcal{L}$ is shorter and it is less probable that a cached content is contained in it. Hence, the parameter $D_{BFS}$ can be used to achieve a trade-off between quality of recommendations (small $D_{BFS}$) and probability of recommending a cached video (large $D_{BFS}$). The number of related videos requested per content $W_{BFS}$, can be interpreted similarly to $D_{BFS}$. A small $W_{BFS}$ leads to considering only top recommendations per video, while a large $W_{BFS}$ leads to a larger~list~$\mathcal{L}$. \blue{For the size of the list $\mathcal{L}$ it holds that 
\[|\mathcal{L}|\leq \sum_{n=1}^{D_{BFS}}(W_{BFS})^{n}\]
where the equality holds when all videos found by the BFS are unique.}

\textit{Remark:} YouTube imposes quotas on the API requests per application per day, which prevents API users from setting the parameters $W_{BFS}$ and $D_{BFS}$ to arbitrarily large values. \blue{However, even with small number of API requests (for related contents), the exploration returns a large number of \textit{unique} videos. Figure~\ref{fig:retVSreq} shows how many relations are requested for parameters $W_{BFS}\in \{1,...,50\}$ and $D_{BFS}=2$ (x-axis), versus the size of the returned list $|\mathcal{L}|$ (y-axis). Two settings are considered, where the BFS starts from a top trending YouTube video from the YouTube ``front page'' or from a video searched through the ``search bar'' (see details in~\secref{sec:measurements}). In both cases the list $\mathcal{L}$ of unique video IDs returned, increases lineraly or almost linearly with the number of explored relations, thus indicating that the BFS achieves an efficient exploration (large $|\mathcal{L}|$) while maintaining a high-quality of recommendations (Table~\ref{table:I-v}).}

\begin{figure}
\centering
\subfigure[``Front Page'' video demand]{\includegraphics[width=0.49\columnwidth]{./figuresSavvas/returnedVSrequested_mostPopular.eps}}
\subfigure[``Search Bar'' video demand]{\includegraphics[width=0.49\columnwidth]{./figuresSavvas/returnedVSrequested.eps}}
\caption{Num. of requested related videos VS Num. of returned related videos from the API.
}
\label{fig:retVSreq}
\end{figure}


%Finally, $N$ affects the probability to recommend both cached and highly related videos (in case they are disjoint sets); e.g., if $N$ is small, the user has a few options, which can promote cached videos but decrease the quality of recommendations.

In practice, \ourAlgo can be fine-tuned through experimentation with real users, e.g., A/B testing iterations, which is a common approach for tuning recommendation systems~\cite{covington2016deep}.

==> System.tex <==
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{./figures/Scheme_1.eps}
\caption{System overview.}
\label{fig:system-overview}
\end{figure}

The proposed approach can be implemented in a lightweight system/application that runs on mobile devices, and is triggered either by the network operator or by the user. The system is composed of the \textit{user interface} (UI), the \textit{back-end}, and the \textit{recommendation module}, as depicted in Fig.~\ref{fig:system-overview}.

\myitem{User Interface (UI).} The UI resembles the original content service UI. For instance, in the YouTube case, the UI contains a search bar, a video player, and a list of related videos\footnote{In the remainder we use the terms \textit{content} and \textit{video} interchangeably.}. The users search, browse, and watch videos through the UI.

\myitem{Back-end.} The back-end is responsible for (i) retrieving the list of cached video IDs (e.g., in the form of a text file), and (ii) streaming videos to the UI. Depending on the scenario, the list of cached video IDs can be already known to the network operator, e.g., in the case of network-controlled caching. Alternatively, they can be requested from the content provider directly\footnote{Note that this refers to an \textit{aggregate} list of the IDs of all the videos stored in a cache, without containing any user information or violating privacy policies.}, or discovered through offline network measurements (e.g., latency~\cite{cache-centric-video-recommendation}, or DNS resolution~\cite{adhikari2011you}) by the network operator. The video requested by the user is delivered/streamed from the CP's (e.g., YouTube's) origin server, or the CP's cache, or an edge cache. In case the caches are controlled by the content provider (which is the most prevalent scenario today), the user-service communication can be encrypted (e.g., https requests directly to YouTube) and remain transparent to the network operator.

%\vassilis{Are you sure that the net provider can easily find out the cached videos? We need to revisit the approach with the DNS queries probably, or propose a Youtube cache-provider interface.}.}

\myitem{Recommendation Module.} The recommendation module is triggered upon each content request, and (i) receives as input the video $v$ that the user currently watches, (ii) retrieves from the YouTube API a list of video IDs directly/indirectly related to $v$, (iii) extracts from the back-end the list of cached video IDs, and (iv) builds a list of \textit{related and cached} video IDs and recommends it to the user, according to the cache-aware recommendation algorithm of \secref{sec:recommendation}. This recommendation process is lightweight and can return the list of recommendations very fast (e.g., $\sim$1sec. in our prototype), without affecting the user experience.
%The recommendation processes are presented in detail in the following section.%Section~\ref{sec:recommendation})


\red{[TODO: check if/how to incorporate] Our goal is not to improve the native YouTube recommender in finding related files, for which it is state of the art, but to use its output as input to our algorithm.}

==> System__BACKUP_20Apr2020.tex <==
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{./figures/Scheme_1.eps}
\caption{System overview.}
\label{fig:system-overview}
\end{figure}

The proposed approach can be implemented in a lightweight system/application that runs on mobile devices, and is triggered either by the network operator or by the user. The system is composed of the \textit{user interface} (UI), the \textit{back-end}, and the \textit{recommendation module}, as depicted in Fig.~\ref{fig:system-overview}.

\myitem{User Interface (UI).} The UI resembles the original content service UI. For instance, in the YouTube case, the UI contains a search bar, a video player, and a list of related videos\footnote{In the remainder we use the terms \textit{content} and \textit{video} interchangeably.}. The users search, browse, and watch videos through the UI.

\myitem{Back-end.} The back-end is responsible for (i) retrieving the list of cached video IDs (e.g., in the form of a text file), and (ii) streaming videos to the UI. Depending on the scenario, the list of cached video IDs can be already known to the network operator, e.g., in the case of network-controlled caching. Alternatively, they can be requested from the content provider directly\footnote{Note that this refers to an \textit{aggregate} list of the IDs of all the videos stored in a cache, without containing any user information or violating privacy policies.}, or discovered through offline network measurements (e.g., latency~\cite{cache-centric-video-recommendation}, or DNS resolution~\cite{adhikari2011you}) by the network operator. The video requested by the user is delivered/streamed from the CP's (e.g., YouTube's) origin server, or the CP's cache, or an edge cache. In case the caches are controlled by the content provider (which is the most prevalent scenario today), the user-service communication can be encrypted (e.g., https requests directly to YouTube) and remain transparent to the network operator.

%\vassilis{Are you sure that the net provider can easily find out the cached videos? We need to revisit the approach with the DNS queries probably, or propose a Youtube cache-provider interface.}.}

\myitem{Recommendation Module.} The recommendation module is triggered upon each content request, and (i) receives as input the video $v$ that the user currently watches, (ii) retrieves from the YouTube API a list of video IDs directly/indirectly related to $v$, (iii) extracts from the back-end the list of cached video IDs, and (iv) builds a list of \textit{related and cached} video IDs and recommends it to the user, according to the cache-aware recommendation algorithm of \secref{sec:recommendation}. This recommendation process is lightweight and can return the list of recommendations very fast (e.g., $\sim$1sec. in our prototype), without affecting the user experience.
%The recommendation processes are presented in detail in the following section.%Section~\ref{sec:recommendation})


\red{[TODO: check if/how to incorporate] Our goal is not to improve the native YouTube recommender in finding related files, for which it is state of the art, but to use its output as input to our algorithm.}

==> realUsers.tex <==
\subsection{Results}
In fig.~\ref{fig:chrcrr-vs-5} we can see that CHR in each video session is analogous to the CRR of the previous video session. For example, in video session 2, we can see that CRR is 67\% (on average) ,  hence 67\% of the contents are cached. As depicted, in video session 2, CHR is 65\%, thus most of the times, users followed cached recommendations. In other words, when we have cached contents inside the Recommendation List, end users are going to follow these recommendations. \newline We also observe that CHR drops, when the video sessions increase in number. This drop in CHR occurs because of the drop in CRR, thus if we optimize our algorithm to provide enough Cached Contents in the Recommendation List, the CHR will maintain high values. 
\newline Fig.~\ref{fig:cd-vs-5} shows what is the probability of picking a cached content, for different CRR values. Users follow a zipf distribution when picking contents from the Recommendation List.
\begin{figure}\centering
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/chrcrrfixed.eps}
\caption{CHR, CRR in 5 consequent video sessions}
\label{fig:chrcrr-vs-5}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/distribs.eps}
\caption{Content Distribution in 5 consequent video sessions}
\label{fig:cd-vs-5}
\end{minipage}
\end{figure}
 


Fig.~\ref{fig:qor-vs-interest} shows that users are interested in the content they picked to watch next from the previous Recommendation List, even if they rated QoR with a lower rating than Interest. 

Fig.~\ref{fig:cdf-vs-interest} shows that users will more probably rate their interest in cached contents with a lower rating than non cached contents. This difference in ratings is not that significant, thus we can say that we have an acceptable trafe off (between interest and chr).
\begin{figure}\centering
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/cdf_intNext_qorPrev.eps}
\caption{QoR with Interest}
\label{fig:qor-vs-interest}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/cdf_interest.eps}
\caption{CDF with Interest}
\label{fig:cdf-vs-interest}
\end{minipage}
\end{figure}
\newline Fig.~\ref{fig:qor-vs-soi-buckets} shows that when QoR is rated with 4 or 5 stars, the average sum of indexes is gathered in an interval of [30, 100] which means that the recommendations are closer to YouTube recommendations. In lower ratings (1, 2, 3) we see that average sums of indexes range in a wider interval, thus CABaRet participates more in the assembly of the RL. We can state that the further we move from YouTube Recommendations, the less probable is for the Recommendation List to be upvoted by the end user. 
\newline Fig.~\ref{fig:int-vs-soi-buckets}  is complementary to Fig.~\ref{fig:qor-vs-soi-buckets} and shows the ratings in interest of an end user for the next video session. 
\begin{figure}\centering
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/qorsoifixed.eps}
\caption{QoR with Sum Of Indexes}
\label{fig:qor-vs-soi}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/intsoi.eps}
\caption{Interest with Sum Of Indexes}
\label{fig:int-vs-soi}
\end{minipage}
\end{figure}

\begin{figure}\centering
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/qorsoibuckets.eps}
\caption{QoR with Sum Of Indexes - Buckets}
\label{fig:qor-vs-soi-buckets}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/intsoibuckets.eps}
\caption{Interest with Sum Of Indexes - Buckets}
\label{fig:int-vs-soi-buckets}
\end{minipage}
\end{figure}

\begin{figure}\centering
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/chrXindex.eps}
\caption{CHR with Index in RL}
\label{fig:chr-vs-index}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/chrXqorXint.eps}
\caption{Cached Probability}
\label{fig:chr-vs-int-qor}
\end{minipage}
\end{figure}

Fig.~\ref{fig:chr-vs-index} shows that 50\% of the times, a user picked a content from the top of the recommendation list. This enhances our assumption that users pick contents from the top-k contents of the RL, thus it is more probable to click on cached content rather than a non-cached.
\newline 



\begin{center}
\begin{tabular}{ c c c }
Ratings & Cached & Non-Cached \\
\hline
QoS & 4.4 & 1.65 \\
\hline
 Interest & 3.45 & 3.6 \\
 \hline
 QoR & 3.4 & 3.55 \\
 \hline
 QoE & 3.5 & 2.1 \\[1ex] 
 \hline
\end{tabular}
\end{center}

\subsection{Methodology}
In our prior work, we assume that the targeted audience is a subset of users that consume contents from recommendation lists. 

Recommendation lists, though, is not the only intermediate for end users to gain access to video contents. Other modules that provide this access are homepages and search bars.
Usually a homepage contains personalized recommendations, thus we can claim that this scenario applies to our prior work. 

The question that raises is: \textbf{ What happens with users that are insensitive in recommendations, and tend to watch videos based on their exact preferences, eg searching a content through a search bar}?



To answer such a question, we need to: 

\begin{itemize}
\item Collect a dataset with the most common keywords that users type into search bars and apply our simulations onto these keywords. In that manner, we can have a holistic understanding on whether our Recommendation System is applicable in today’s Video Streaming Ecosystem
\item To get a large and representative corpus of YouTube video catalog, we use the YouTube data API and search YouTube with specific keywords obtained from Google Top Trends website. Specifically, we use around 4k keywords extracted from the top charts for each month from early 2015 to November 2017
\item For each keyword, we collect the top 10 video IDs returned from YouTube API, resulting into ~40k unique Video IDs
\item We feed the simulation script with each and every Video ID and we extract the average CHR achieved after 5 simulation steps
\item After processing, we build a dataset of around X entries for Y unique video keywords
\item Each entry in this dataset represents a unique video identified by a video ID and the CHR achieved by using this Video ID as seed to the simulation script
\end{itemize}

\begin{figure}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/googleTrends/fig_CHR_vs_probabilityGR.eps}
\caption{(cached = mp) CHR under different BFS parameters (Search)}
\label{fig:searchListResults}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/googleTrends/fig_CHR_vs_cacheSizeGR.eps}
\caption{(cached = mp) CHR vs \# cached contents C (Wbfs = 50, Dbfs = 2).}
\label{fig:searchListResults2}
\end{minipage}
\end{figure}



\begin{figure}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/googleTrends/fig_CHR_vs_cacheSizeGR_cachedMostSearched.eps}
\caption{(cached = ms) CHR vs \# cached contents C (Wbfs = 50, Dbfs = 2).}
\label{fig:searchListResults3}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/googleTrends/fig_CHR_vs_probabilityGR_cachedMostSearched.eps}
\caption{(cached = ms) CHR under different BFS parameters (Search)}
\label{fig:searchListResults4}
\end{minipage}
\end{figure}









\begin{figure}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/cacheSizeSearchUniform.eps}
\caption{CHR vs \# cached contents C (pi = uniform, Wbfs = 50, Dbfs = 2).}
\label{fig:greedyCachingUni}
\end{minipage}
\begin{minipage}[t]{0.46\linewidth}
\centering
\includegraphics[width=1\columnwidth]{./figuresSavvas/cacheSizeSearchZipf1.eps}
\caption{CHR vs \# cached contents C (pi = zipf1, Wbfs = 50, Dbfs = 2).}
\label{fig:greedyCachingZipf1}
\end{minipage}
\end{figure}




\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{./figuresSavvas/googleTrends/cacheSizeSearchZipf1US.eps}
\caption{US-CHR vs \# cached contents C (pi = zipf1, Wbfs = 50, Dbfs = 2).}
\label{fig:greedyCachingUniUS}
\end{figure}
